Exploring home robot capabilities by medium fidelity prototyping

In order for autonomous robots to be able to support people's well-being in homes and everyday environments, new interactive capabilities will be required, as exemplified by the soft design used for Disney's recent robot character Baymax in popular fiction. Home robots will be required to be easy to interact with and intelligent--adaptive, fun, unobtrusive and involving little effort to power and maintain--and capable of carrying out useful tasks both on an everyday level and during emergencies. The current article adopts an exploratory medium fidelity prototyping approach for testing some new robotic capabilities in regard to recognizing people's activities and intentions and behaving in a way which is transparent to people. Results are discussed with the aim of informing next designs.

==> Makefile <==
TEX = acmsmall-sample.tex \
	sample10.tex \
	sample11.tex \
	sample1.tex \
	sample2.tex \
	sample3.tex \
	sample4.tex \
	sample5.tex \
	sample6.tex \
	sample7.tex \
	sample8.tex \
	sample9.tex \


CLS = acmsmall.cls

STY = acmcopyright.sty

PACKAGE = acmsmall

PDF = ${TEX:%.tex=%.pdf} acm-update.pdf

PWD= ${shell pwd}

all: $(PDF)

%.pdf: %.tex $(CLS) $(STY)
	pdflatex $*
	bibtex $*
	pdflatex $*
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log)\
	do pdflatex $*; done

acm-update.pdf:  ../documentation/acm-update.tex
	cd ../documentation; ${MAKE}; cd ${PWD}; cp ../documentation/$@ .

acmcopyright.sty:  ../acmcopyright/acmcopyright.dtx
	cd ../acmcopyright; ${MAKE}; cd ${PWD}; cp ../acmcopyright/$@ .

clean:
	$(RM) *.aux *.log  *.blg

distclean: clean
	$(RM) $(PDF) acm-update.pdf *.bbl

zip: all clean
	zip $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'
